GMCR: Graph-based Maximum Consensus Estimation for Point Cloud Registration

Point cloud registration is a fundamental and challenging problem for autonomous robots interacting in unstructured environments for applications such as object pose estimation, simultaneous localization and mapping, robot-sensor calibration, and so on. In global correspondence-based point cloud registration, data association is a highly brittle task and commonly produces high amounts of outliers. Failure to reject outliers can lead to errors propagating to downstream perception tasks. Maximum Consensus (MC) is a widely used technique for robust estimation, which is however known to be NP-hard. Exact methods struggle to scale to realistic problem instances, whereas high outlier rates are challenging for approximate methods. To this end, we propose Graph-based Maximum Consensus Registration (GMCR), which is highly robust to outliers and scales to realistic problem instances. We propose novel consensus functions to map the decoupled MC-objective to the graph domain, wherein we find a tight approximation to the maximum consensus set as the maximum clique. The final pose estimate is given in closed-form. We extensively evaluated our proposed GMCR on a synthetic registration benchmark, robotic object localization task, and additionally on a scan matching benchmark. Our proposed method shows high accuracy and time efficiency compared to other state-of-the-art MC methods and compares favorably to other robust registration methods.

==> figures/3_method/fgreg_pseudo_code.tex <==
\begin{algorithm}[t!]
  \SetAlgoLined
  \small
  \KwData{source points $\mathcal{A}$, target points $\mathcal{B}$, corresp. $\mathcal{C}$, noise bounds $\boldsymbol{\beta}$, cutoff $c$}
  \KwResult{scale $\hat{s}$, rotation $\hat{\mathbf{R}}$, translation $\hat{\mathbf{t}}$}
  \tcp{Compute invariants}
  $\mathcal{A}_c \leftarrow \mathcal{A}[\mathcal{C}[:, 0]]$, $\mathcal{B}_c \leftarrow \mathcal{B}[\mathcal{C}[:, 1]]$ \;
  $\Bar{\mathcal{A}}, \Bar{\mathcal{B}}, \boldsymbol{\delta} \leftarrow$ compute\_tims($\mathcal{A}_c$, $\mathcal{B}_c$, $\boldsymbol{\beta}$) \Comment*[r]{eq. \ref{eq:corresp_est:tims}\phantom{0}}
  $\Bar{\Bar{\mathcal{A}}}, \Bar{\Bar{\mathcal{B}}}, \boldsymbol{\alpha} \leftarrow$ compute\_trims($\Bar{\mathcal{A}}$, $\Bar{\mathcal{B}}$, $\boldsymbol{\delta}$) \Comment*[r]{eq. \ref{eq:corresp_est:trims}}

  \uIf{estimate\_scale}{
      \tcp{Scale estimation}
      $\mathcal{G}_s \leftarrow $ scale\_consensus($\Bar{\Bar{\mathcal{A}}}$, $\Bar{\Bar{\mathcal{B}}}$, $\boldsymbol{\alpha}$, $c$) \Comment*[r]{eq. \ref{eq:consensus:scale}}
      $\mathcal{I}_s \leftarrow $ max\_clique($\mathcal{G}_s$)  \;
      $\hat{s} \leftarrow $ compute\_scale($\mathcal{I}_s$) \Comment*[r]{eq. \ref{eq:corresp_est:scale_obj}}
      $\Bar{\mathcal{A}} \leftarrow \hat{s} \cdot \Bar{\mathcal{A}} $ \;
  }
  \Else{
    \tcp{Scale Outlier Pruning}
    $\mathcal{G}_c \leftarrow$ scale\_consistency($\Bar{\Bar{\mathcal{A}}}, \Bar{\Bar{\mathcal{B}}}, \boldsymbol{\alpha}, c$) \;
    $\mathcal{I}_c \leftarrow$ max\_clique($\mathcal{G}_c$) \;
    $\mathcal{A}_c, \mathcal{B}_c \leftarrow \mathcal{A}_c[\mathcal{I}_c], \mathcal{B}_c[\mathcal{I}_c]$ \;
    $\Bar{\mathcal{A}}_c, \Bar{\mathcal{B}}_c \leftarrow \Bar{\mathcal{A}}_c[\mathcal{I}_c], \Bar{\mathcal{B}}_c[\mathcal{I}_c]$ \;    
  }

  \tcp{Rotation estimation}
  $\mathcal{G}_R \leftarrow$ rotation\_consensus($\Bar{\mathcal{A}}$, $\Bar{\mathcal{B}}$, $\boldsymbol{\delta}$, $c$) \Comment*[r]{eq. \ref{eq:consensus:rotation}}
  $\mathcal{I}_R \leftarrow $ max\_clique($\mathcal{G}_R$) \;
  $\hat{\mathbf{R}} \leftarrow$ compute\_rotation($\mathcal{I}_R$) \Comment*[r]{eq. \ref{eq:obj_trans_decoupled}}
  \tcp{Translation estimation}
  $\mathcal{A}_c \leftarrow \hat{s} \hat{\mathbf{R}} \cdot \mathcal{A}_c$ \;
  $\mathcal{G}_t \leftarrow$ translation\_consensus($\mathcal{A}_c$, $\mathcal{B}_c$, $\boldsymbol{\beta}$, $c$) \Comment*[r]{eq. \ref{eq:corresp_est:translation_consensus_funct}}
  $\mathcal{I}_t \leftarrow $ max\_clique($\mathcal{G}_t$) \; 
  $\hat{\mathbf{t}} \leftarrow $ compute\_translation($\mathcal{I}_t$) \Comment*[r]{eq. \ref{eq:pcr_maxcon}\phantom{0}}
  \caption{Our Graph-based Registration Framework}
  \label{algorith:fg_reg}
\end{algorithm}



==> results/3d_match_images.tex <==
\begin{figure}[h!]
\begin{subfigure}[b]{.49\linewidth}
  \centering
  \includegraphics[width=\linewidth]{ICRA_2023/results/3d_match_results/3d_match_1_new.png}
  \caption{Before}
  \label{fig:3dmatch_1}
\end{subfigure}
\begin{subfigure}[b]{.49\linewidth}
  \centering
  \includegraphics[width=\linewidth]{ICRA_2023/results/3d_match_results/3d_match_2.png}
  \caption{Aligned}
  \label{fig:3dmatch_2}
\end{subfigure}
\caption{Sample from \textit{3DMatch}\cite{zeng20163dmatch} dataset with putative correspondences shown in orange (left) and registration result (right).}
\label{fig:scene_matching_image}
\end{figure}

==> results/ablations_figure.tex <==
\begin{figure*}[t!]
\begin{subfigure}[c]{.24\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{results/ablation_plots/ablation_scale.png}
  \caption{Scale}
  \label{fig:ablation_scale}
\end{subfigure}
\begin{subfigure}[c]{.24\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{results/ablation_plots/ablation_rotation.png}
  \caption{Rotation}
  \label{fig:ablation_rotation}
\end{subfigure}
\begin{subfigure}[c]{.24\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{results/ablation_plots/ablation_translation.png}
  \caption{Translation}
  \label{fig:ablation_translation}
\end{subfigure}
\begin{subfigure}[c]{.24\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{results/ablation_plots/ablation_graph_deg.png}
  \caption{Graph degeneracy}
  \label{fig:ablation_graph_deg}
\end{subfigure}\hfill
\caption{Analysis of inlier distributions in scale, rotation and translation \textit{Fitting Graphs} in a) - c). Graph degeneracy for those consensus functions in d).}
\label{fig:ablations}
\end{figure*}

==> results/lin_reg_plot.tex <==
\begin{figure*}[t!]
\begin{subfigure}[c]{.24\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{ICRA_2023/results/lin_reg/linreg_plot_1.png}
  %\caption{}
  \label{fig:lin_reg_gt}
\end{subfigure}
\begin{subfigure}[c]{.24\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{ICRA_2023/results/lin_reg/linreg_plot_2.png}
  %\caption{}
  \label{fig:lin_reg_ls}
\end{subfigure}
\begin{subfigure}[c]{.24\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{ICRA_2023/results/lin_reg/linreg_plot_3.png}
  %\caption{}
  \label{fig:lin_reg_rans}
\end{subfigure}
\begin{subfigure}[c]{.24\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{ICRA_2023/results/lin_reg/linreg_plot_4.png}
  %\caption{}
  \label{fig:lin_reg_fg}
\end{subfigure}\hfill
\caption{Robust linear regression on toy dataset.}
\label{fig:lin_reg}
\end{figure*}

==> results/nuscenes_results/nuscenes_table_mean.tex <==
\begin{table}[]
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{@{}llll@{}}
\toprule
         & \multicolumn{1}{c}{$R$} & \multicolumn{1}{c}{$t$} & \multicolumn{1}{c}{\%} \\ \midrule
FGR      & $44.05\pm 59.53$        & $2.15 \pm 2.83$         & $49$                   \\
TEASER++ & $8.25 \pm 32.91$        & $0.45 \pm 1.59$         & $92$                   \\ \midrule
Ours     & $5.32 \pm 22.80$        & $0.35 \pm 1.45$         & $95$                   \\ \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Results on NuScenes-mini lidar scan matching benchmark}
\end{table}

==> results/nuscenes_results/nuscenes_table_old.tex <==
\begin{table*}[]
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lllllllllllll}
\hline
         & \multicolumn{3}{c}{N=1}                                                    & \multicolumn{3}{c}{N=2}                                                    & \multicolumn{3}{c}{N=3}                                                    & \multicolumn{3}{c}{N=4}                                                    \\ \hline
         & \multicolumn{1}{c}{$R$} & \multicolumn{1}{c}{$t$} & \multicolumn{1}{c}{\%} & \multicolumn{1}{c}{$R$} & \multicolumn{1}{c}{$t$} & \multicolumn{1}{c}{\%} & \multicolumn{1}{c}{$R$} & \multicolumn{1}{c}{$t$} & \multicolumn{1}{c}{\%} & \multicolumn{1}{c}{$R$} & \multicolumn{1}{c}{$t$} & \multicolumn{1}{c}{\%} \\ \hline
FGR      & $44.05\pm 59.53$        & $2.15 \pm 2.83$         & $49$                   & $50.98 \pm 63.14$       & $3.77 \pm 4.81$         & $46$                   & $56.17 \pm 63.46$       & $6.50 \pm 7.35$         & $40$                   & $54.99 \pm 62.60$       & $7.82 \pm 9.26$         & $41$                   \\
TEASER++ & $8.25 \pm 32.91$        & $0.45 \pm 1.59$         & $92$                   & $20.14 \pm 49.10$       & $1.89 \pm 4.34$         & $83$                   & $32.84 \pm 59.74$       & $4.02\pm 7.06$          & $69$                   & $43.81\pm 65.61$        & $6.84 \pm 9.95$         & $58$                   \\ \hline
Ours     & $5.32 \pm 22.80$        & $0.35 \pm 1.45$         & $95$                   & $19.45 \pm 44.77$       & $1.95 \pm 4.31$         & $80$                   & $31.72 \pm 55.10$       & $4.22 \pm 7.29$         & $70$                   & $42.96 \pm 61.73$       & $7.05 \pm 10.15$        & $60$                   \\ \hline
\end{tabular}
\end{adjustbox}
\end{table*}

==> results/obj_loc_images.tex <==
\begin{figure*}
\centering
\begin{minipage}[h]{.8\textwidth}
\centering
\begin{subfigure}[b]{.19\linewidth}
  \centering
  \includegraphics[width=\linewidth]{ICRA_2023/results/obj_loc_results/bowl_1_new.png}
  %\caption{Scale}
  \label{fig:obj_bowl_1}
\end{subfigure}\hfill
\begin{subfigure}[b]{.19\linewidth}
  \centering
  \includegraphics[width=\linewidth]{ICRA_2023/results/obj_loc_results/cap_1_new.png}
  %\caption{Rotation}
  \label{fig:obj_cap_1}
\end{subfigure}\hfill
\begin{subfigure}[b]{.19\linewidth}
  \centering
  \includegraphics[width=\linewidth]{ICRA_2023/results/obj_loc_results/cereal_box_1_new.png}
  %\caption{Translation}
  \label{fig:obj_cereal_box_1}
\end{subfigure}\hfill
\begin{subfigure}[b]{.19\linewidth}
  \centering
  \includegraphics[width=\linewidth]{ICRA_2023/results/obj_loc_results/coffee_mug_1_new.png}
  %\caption{Graph degeneracy}
  \label{fig:obj_coffee_mug_1}
\end{subfigure}\hfill
\begin{subfigure}[b]{.19\linewidth}
  \centering
  \includegraphics[width=\linewidth]{ICRA_2023/results/obj_loc_results/soda_can_1_new.png}
  %\caption{Graph degeneracy}
  \label{fig:obj_soda_can_1}
\end{subfigure}\hfill
\begin{subfigure}[b]{.19\linewidth}
  \centering
  \includegraphics[width=\linewidth]{ICRA_2023/results/obj_loc_results/bowl_2_new.png}
  \caption{\textit{bowl}}
  \label{fig:obt_bowl_2}
\end{subfigure}\hfill
\begin{subfigure}[b]{.19\linewidth}
  \centering
  \includegraphics[width=\linewidth]{ICRA_2023/results/obj_loc_results/cap_2_new.png}
  \caption{\textit{cap}}
  \label{fig:obj_cap_2}
\end{subfigure}\hfill
\begin{subfigure}[b]{.19\linewidth}
  \centering
  \includegraphics[width=\linewidth]{ICRA_2023/results/obj_loc_results/cereal_box_2_new.png}
  \caption{\textit{cereal\_box}}
  \label{fig:obj_cereal_box_2}
\end{subfigure}\hfill
\begin{subfigure}[b]{.19\linewidth}
  \centering
  \includegraphics[width=\linewidth]{ICRA_2023/results/obj_loc_results/coffee_mug_2_new.png}
  \caption{\textit{coffee\_mug}}
  \label{fig:obj_coffee_mug_2}
\end{subfigure}\hfill
\begin{subfigure}[b]{.19\linewidth}
  \centering
  \includegraphics[width=\linewidth]{ICRA_2023/results/obj_loc_results/soda_can_2_new.png}
  \caption{\textit{soda\_can}}
  \label{fig:obj_soda_can_2}
\end{subfigure}\hfill
\caption{Object localization results on the \textit{RGB-D Dataset}. Putative correspondences are shown in orange and the object is shown in blue.}
\label{fig:object_loc_images}
\end{minipage}
\end{figure*}


==> results/object_localization_table.tex <==
\begin{table}[b!]
\begin{center}
\caption{Object localization on the \textit{RGB-D Dataset}\cite{Lai} in median and median absolute deviation.}
\label{tab:object_loc}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}ccccc@{}}
    \hline
    \textbf{Object} & \textbf{Method} & $\mathbf{R} [deg]$ & $\mathbf{t} [cm]$ & $\%$ \\
    \hline
    \multirow{3}{*}{\textit{bowl}} & RANSAC & $129.23 \pm 37.30$ & $168.05 \pm 100.22$ & $6.7$ \\
    &TEASER++ & $\mathbf{4.67\pm 3.77}$ & $\mathbf{4.65 \pm 3.57}$  & $\mathbf{60}$ \\
    %\cdashline{2-5}
    &FGREG (Ours) & $10.271 \pm 7.75$ & $10.70 \pm 8.14$ & $47$ \\
    \hline
    \multirow{3}{*}{\textit{cap}} & RANSAC & $117.21 \pm 35.24$ & $204.6 \pm 62.50$ & $0$ \\
    &TEASER++ & $6.47 \pm 3.82$ & $5.36 \pm 3.17$ & $67$\\\
    % \cdashline{2-5}
    &FGREG (Ours) & $\mathbf{2.23 \pm 1.09}$ & $\mathbf{3.04 \pm 1.77}$ & $\mathbf{83}$\\
    \hline
    \multirow{3}{*}{\textit{cereal\_box}} & RANSAC & $125.47 \pm 25.51$ & $171.41 \pm 85.76$ & $13$ \\
    &TEASER++ & $2.17 \pm 1.35$ & $\mathbf{2.15 \pm 1.73}$ & $\mathbf{87}$ \\
    %\cdashline{2-5}
    &FGREG (Ours) & $\mathbf{1.98 \pm 1.50}$ & $3.84 \pm 2.63$ & $73$ \\
    \hline
    \multirow{3}{*}{\textit{coffee\_mug}} & RANSAC & $129.16 \pm 26.08$ & $277.02 \pm 85.45$ & $0$ \\
    &TEASER++ & $8.12 \pm 7.74$ & $8.63 \pm 8.23$ & $50$ \\
    %\cdashline{2-5}
    &FGREG (Ours) & $\mathbf{2.39 \pm 2.10}$ & $\mathbf{2.52 \pm 2.14}$ & $\mathbf{75}$ \\
    \hline
    \multirow{3}{*}{\textit{soda\_can}} & RANSAC & $115.06 \pm 37.42$ & $452.62 \pm 178.49$ & $6$ \\
    &TEASER++ & $14.89 \pm 13.05$ & $22.81 \pm 19.67$ & $28$ \\
    %\cdashline{2-5}
    &FGREG (Ours) & $\mathbf{4.43 \pm 2.70}$ & $\mathbf{4.64 \pm 2.07}$ & $\mathbf{67}$ \\
    \hline
\end{tabular}}
\end{center}
\end{table}

==> results/scan_matching_table.tex <==
\begin{table}[t!]
\begin{center}
\caption{Registration results on the \textit{3DMatch}\cite{zeng20163dmatch} dataset. Results are given in median and median absolute deviation.}
\label{tab:scan_matching}
\begin{tabular}{@{}ccccc@{}}

Method & $\mathbf{R} [deg]$ & $\mathbf{t} [m]$ & $\%$   \\
         \cline{1-4}
RANSAC   &  $113.732 \pm 42.802$ & $2.419 \pm 0.940$             &  $0$          \\
TEASER++ &   $\mathbf{2.378 \pm 1.242}$& $0.395 \pm 0.337$ & $44.3$      \\
% \hline
FGREG    & $2.784 \pm 1.429$ & $\mathbf{0.379 \pm 0.306}$ & $\mathbf{45.7}$   \\
\hline
\end{tabular}
\end{center}
\end{table}

==> sections/related_work.tex <==
\section{Related Work}\label{sec:related_work}
\todo[inline]{Start with robust registration methods, also talk about preprocessing / pure outlier removal methods and finish with maximum consensus}

Point cloud registration is the process of finding the rigid transformation (scale, rotation, and translation) that aligns two point sets. One line of work first estimates correspondences and then solves the registration. If reliable correspondences are known, the transformation can be extracted in closed form~\cite{Horn1987, Arun1987}. However, as correspondence estimation is prone to errors and usually produces high outlier rates\cite{Bustos2018}, robust registration approaches were developed. \textit{Olsson et al.}~\cite{Olsson2009} proposed a Branch-and-Bound (BnB) optimization framework, which is then used for rigid registration. \textit{Briales et al.}~\cite{Briales} extended this formulation with a tight semidefinite relaxation. One of the earliest robust estimation methods that is still widely used today, is Random Sample Consensus (RANSAC)~\cite{fischler1981random}. However, RANSAC convergence degenerates when a large number of outliers is present~\cite{Bustos2018}. 
% \textit{MacTavish and Barfoot} \cite{MacTavish2015} showed that an aggressively redescending cost, like the \textit{Geman-McClure} or \textit{Dynamic Covariance Scaling} best removes outliers. 
\textit{Zhou et al.}~\cite{Zhou2016} proposed Fast Global Registration (FGR) where Black-Rangarajan duality was used to simplify the robust estimation problem into a line process, which was then solved using Graduated Non-convexity (GNC).
% \textit{Enqvist et al.} \cite{Enqvist2009} developed the notion of consistency graphs, where the scale is used as consistency measure and the inlier set is then obtained from the vertex cover problem.
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{RAL-IROS_2022/figures/1_introduction/first_figure.png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}
\textit{Bustos et al.}~\cite{Bustos2018} proposed Guaranteed Outlier Removal (GORE), which is proven to only remove true outliers. In GORE, geometric operations were used to compute lower and upper bounds on the Maximum Consensus set and the transformations were extracted using \textit{BnB}.
% For general transformations, \textit{GORE} relies on \textit{BnB}. 
% \textit{Parra et al.}\cite{Parra2019a} introduced a graph-based formulation for rejecting outliers, which is similar to \textit{Enqvist et al.}\cite{Enqvist2009}. Distances between pairs of correspondences were used to build a graph, where a \textit{Practical Maximum Clique (PMC)} algorithm was then proposed to reject outliers. \textit{Yang and Carlone} used a \textit{Truncated least-squares (TLS)} cost function, to solve the registration problem robustly in \cite{Yang2019a}. Scale and translation estimation was solved using a version of \textit{1-point-RANSAC} \cite{Scaramuzza2011} termed \textit{Adaptive Voting}, whereas rotation leveraged a semi-definite relaxation. The rotation estimation formulation was then extended in \cite{Yang2019} using quaternions, to obtain a certificate of the obtained solution.
\textit{Yang et al.}~\cite{Yang2021} proposed TEASER++ which uses \textit{Truncated-Least-Squares (TLS)} to robustly solve the registration problem in presence of high outlier rates and provide theoretical bounds on the estimation errors.
% By adding extensive outlier rejection and introducing algorithmic advances, those works were combined in \textit{TEASER} \cite{Yang2021}. 
% This concept using \textit{TLS} was then generalized \cite{Yang2020a} to a wide range of perception problems, wherein the \textit{TLS} was reformulated to an optimization over \textit{Lasserre's Hierarchy of Convex Moment Relaxations}.
% \textit{Antonante et al.} \cite{Antonante2020} developed two new general formulations for \textit{Maximum Consensus} and \textit{Truncated least-squares (TLS)}, wherein a novel technique is used to dynamically set the outlier thresholds. Recently graph-based outlier rejection methods, based on consistency graphs \cite{Parra2019a}, have been adopted.
\textit{Shi et al.}~\cite{Shi2020} proposed ROBIN, which is a consistency-graph-based outlier removal method using invariants, which finds an approximation to the maximum clique problem using the k-core. CLIPPER~\cite{Lusk2021} advanced this work, by introducing a novel relaxation for the \textit{Maximum Clique} problem. The relaxation is fast and even tight for weighted graphs. Consistency-graph-based methods however require a known quantity, such as scale, to prune outliers. \textit{Lin et al.}\cite{lin2022closest} propose an efficient consistency-graph-based method to reduce the computational complexity of correspondence based methods, such as \textit{TEASER++}\cite{Yang2021}. Also inspired from~\cite{Shi2020}, \textit{Sun et al.}~\cite{Sun2021} proposed RANSIC wherein a RANSAC-based approach was developed which used simple checks performed on minimal subsets of measurements to find the maximum consensus set. In contrast to correspondence-based methods, simultaneous pose and correspondence methods (SPC) solve the correspondence estimation and registration problems jointly. Local methods, like Iterative Closest Point (ICP)~\cite{Besl1992} and its robust extensions \cite{Granger2002, Kaneko2003, Chetverikov2005, Maier-Hein2012} are not guaranteed to find a global optimum and are susceptible to local minima~\cite{Yang2021}. 
% \textit{Myronenko et. al.} \cite{Myronenko2010} used a \textit{Gaussian Mixture Model (GMM)} to solve the rigid registration problem, which represents one point set and is assumed to have generated the other point set. \textit{Jian et. al.}\cite{Jian2011} also adopted \textit{GMMs}, but fitted a model to each point set and then matched components. \textit{Clark et. al.} \cite{Clark2020} defined a continuous function for the raw measurements, which is then aligned using the lie group. \textit{Le et al.}\cite{Le} use graph matching in a RANSAC-Framework, where the matching potential is given by the difference in length for a pair of correspondences. Global SPC methods integrate the alternating optimization into a global optimization framework. \textit{Breuel et al.} \cite{Breuel2003} introduced a general match-list based \textit{BnB} approach, that has wide applications in perception. \textit{Hertley et al.} \cite{Hartley2009} used a \textit{BnB} approach for rotation search. It covers the whole rotation space and therefore guarantees a globally optimal solution. To increase the search speed \textit{Bustos et al.} \cite{ParraBustos2016} introduced a novel bounding function.
\textit{Yang et al.}~\cite{Yang2016} proposed a globally optimal ICP variant termed Go-ICP. They extended BnB to the domain of $SE(3)$ and incorporated an ICP approach. Recently, \textit{Murali et al.}~\cite{murali2021active, murali2022active} proposed a translation-invariant quaternion filter (TIQF) which is a filtering-based approach for registration applicable to both dense and sparse point sets.  
% \cite{Maron2016} focused on the \textit{Procrustes Matching (PM)} problem, of which the \textit{SPC} problem is a particular instance, and used a \textit{Semi-Definite} relaxation to make it tractable. \textit{Izatt et al.} \cite{Izatt2020} formulate it as a \textit{Mixed-Integer-Liner-Program(MILP)}, which is then solved with a BnB-Solver. 
% \paragraph{Deep Learning based Methods}
On the other hand, deep-learning proved to be very effective and efficient in the domain of 3D point sets~\cite{guo2020deep}. \textit{Aoki et al.}~\cite{Aoki2019} introduced \textit{PointNetLK}, which was based on the PointNet architecture~\cite{Qi2017} and uses the Lukas-Kanade method to minimize the feature re-projection error. \textit{Wang et al.}~\cite{Wang2019a} proposed Deep Closest Point (DCP) wherein features from a Dynamic Graph CNN (DGCNN)~\cite{Wang2019b} and a transformer are used to estimate correspondences, which are then used to solve the registration.
% \textit{PRNet}\cite{Wang2019} extended \textit{DCP} for partial scans, where part of the shape is occluded. \textit{Avetisyan et al.}\cite{Avetisyan2019a} tackled the problem of aligning CAD models with 3D scans represented by \textit{Signed-Distance-Functions (SDF)}. A 3D CNN-based correspondence estimation network was used to find soft matches and registration was then performed using the \textit{Levenberg-Marquardt} algorithm. This was extended \cite{Avetisyan2019} using a differentiable \textit{Procrustes} alignment loss and symmetry aware correspondence prediction. \textit{Gojcic et al.} \cite{Gojcic2019} introduced \textit{3DSmoothNet}, producing strong rotation-invariant features. Together with a RANSAC-Framework they can be used for registration. \textit{Deep Global Registration} \cite{Choy2020} uses \textit{Fully Convolutional Geometric Features (FCGF)} \cite{Choy2019} to predict correspondence confidences. The registration is solved in a $SE(3)$ procrustes formulation.
%%%%%%%%%%%

\subsection{Robust Registration}

\subsection{Maximum Consensus Estimation}


\begin{remark}[On relation to other graph-based methods]
CLIPPER \cite{Lusk2021}, ROBIN \cite{Shi2020} and PMC\cite{Parra2019a} address the task of matching with pairwise constrains. Therein associations are represented by nodes and edges are present, if two associations are consistent. In those consistency or compatibility graphs the maximum clique represents the largest set of associations that are pairwise consistent and thus the inlier set. In our proposed formulation the nodes are measurements (scale, rotation or translation) and edges encode consensus, i.e. an edge is present if two measurements are in at least one consensus set together. Therefore the maximum clique in our graph encodes the maximum consensus estimate. Thus we perform robust estimation using a graph-based formulation. 
\cite{Enqvist2009}

\end{remark}
